Prescribed Fire Modeling using Knowledge-Guided Machine Learning for Land Management

In recent years, the increasing threat of devastating wildfires has underscored the need for effective prescribed fire management. Process-based computer simulations have traditionally been employed to plan prescribed fires for wildfire prevention. However, even simplified process models like QUIC-Fire are too compute-intensive to be used for real-time decision-making, especially when weather conditions change rapidly. Traditional ML methods used for fire modeling offer computational speedup but struggle with physically inconsistent predictions, biased predictions due to class imbalance, biased estimates for fire spread metrics (e.g., burned area, rate of spread), and generalizability in out-of-distribution wind conditions. This paper introduces a novel machine learning (ML) framework that enables rapid emulation of prescribed fires while addressing these concerns. By incorporating domain knowledge, the proposed method helps reduce physical inconsistencies in fuel density estimates in data-scarce scenarios. To overcome the majority class bias in predictions, we leverage pre-existing source domain data to augment training data and learn the spread of fire more effectively. Finally, we overcome the problem of biased estimation of fire spread metrics by incorporating a hierarchical modeling structure to capture the interdependence in fuel density and burned area. Notably, improvement in fire metric (e.g., burned area) estimates offered by our framework makes it useful for fire managers, who often rely on these fire metric estimates to make decisions about prescribed burn management. Furthermore, our framework exhibits better generalization capabilities than the other ML-based fire modeling methods across diverse wind conditions and ignition patterns.

==> intro.tex <==
% Neural Style Transfer is a popular computer vision technique that enables reconstruction of images and videos that closely represents reference style provided as input to the model. While this method has been extensively used in computer vision, this methodology elusive in physics-guided machine learning. In our use case, we enable style transfer in terms of different ignition patterns, wind speed and wind direction scenarios. %domain adaptation, entity-aware learning

% "One way for domain adaption is to match a sample in the source domain to that in the target domain by minimising their distribution discrepancy, in which Maximum Mean Discrepancy (MMD) is a popular choice to measure the discrepancy between two
% distributions. Li et al. prove that matching Gram-based style representations between a pair of style and stylised images is
% for MMD can be equally applied in NST"



Thousands of wildfires engulf millions of acres in the United States each year alone \cite{abatzoglou2016impact}. These fires threaten wildlife and human lives and destroy personal property.  A prescribed fire, also called a prescribed burn, is the intentional and controlled lighting of fire that is ignited only when specific conditions are met to ensure fire crews can manage the fire's spread and achieve the management burn's objectives. Burn bosses (or fire managers) use prescribed fires to reduce the fuel that feeds extreme fires and help improve forest health by recycling soil nutrients and controlling pests \cite{wiedinmyer2010prescribed, hiers2020prescribed}. Factors like wind speed and direction, the region's topography, surface moisture, and fuel characteristics all impact the fire behavior of prescribed burns. 

\begin{figure}[h]
    \centering
    % \includegraphics[width=0.30\textwidth]{images/intro/physics_guided_emulator.eps}
    \includegraphics[width=0.47\textwidth]{images/intro/PGCLplus-v2.png}
    % \vspace{-10pt}
    \caption{Physics-guided Emulator for fuel density estimation. Inputs include source fuel density, ignition pattern, initial wind speed, and initial wind direction.}
    \label{fig:model-diagram}
    \vspace{-10pt}
\end{figure}

Historically, process-based models have provided pathways for simulating the physical processes in a fire system \cite{jain2020review}. However, of all the process-based models, QUIC-Fire is the only one specifically designed for prescribed fire simulation  \cite{linn2020quic}.
QUIC-Fire (QF) is a fast-running and inexpensive computational tool, providing significant speedup over other process-based models \cite{gallagher2021reconstruction}. QUIC-Fire is able to represent complex fire atmospheric interactions and fireline interactions, making it suitable to use when investigating the effect of ignition patterns on fire behavior.  However, despite the success of QUIC-Fire, its computation time and resource requirements still limit its usability for real-time decision-making, which may be pivotal for ensuring the safety of firefighters and making rapid assessments of fire spread under changing weather conditions.

While machine learning (ML) provides an avenue for fast predictions that can be useful for operational prescribed burn planning, current machine learning frameworks predominantly focus only on wildfire modeling \cite{toulouse2017computer}. Due to several differences in the exogenous variables, ignition patterns, and fire spread mechanisms, methods developed for wildfires are not suitable for modeling prescribed fires. Wildfires and prescribed fires differ in their physical behavior and environmental conditions, with wildfires being accidental, long-lasting fires ignited under low moisture and higher wind speeds, while prescribed fires are intentionally set by burn bosses under controlled conditions, often involving multiple fire lines interacting with each other. The current state of ML methods for prescribed burns primarily focuses on post-burn modeling objectives, such as burn detection \cite{cope2021using, agastra2020evaluating, perez2020evaluation} and smoke management \cite{afrin2021machine}. However, there is still a need for a framework that can be useful in pre-burn real-time identification of safe conditions for prescribed fires.

% Machine learning (ML) methods present an opportunity for fast predictions that can be useful in immediate prescribed burn planning.  However, machine learning (ML) models developed for studying fire systems predominantly focus only on wildfire modeling \cite{toulouse2017computer}, which have very different physical behavior than prescribed fires. This difference arises due to the differences in environmental conditions under which fires start. Wildfires are accidental fires that start under low moisture and higher wind speeds and burn for longer time periods. In contrast, prescribed fires are lit by burn bosses under lower wind speed conditions and controlled environmental conditions. Moreover, prescribed fires are often ignited as multiple fire lines that interact with each other, creating a more complex physical system for modeling. Very few ML methods study prescribed fires \cite{cope2021using} - the majority of them focus on fire detection \cite{agastra2020evaluating}, burn severity \cite{perez2020evaluation}, and smoke management \cite{afrin2021machine}. However, for real-time prescribed fire planning, burn bosses require access to time-series forecasts of the prescribed fire evolution - which is not achieved by the modeling objectives addressed in previous studies and will be the problem we address in this paper. Furthermore, the lack of real-world input datasets for prescribed burns further exacerbates the problem \cite{gallagher2021reconstruction, linn2020quic}. This limits the usage of traditional ML models in scenarios where large-scale datasets are not available for training the model. 

% Machine learning (ML) methods present an opportunity for fast predictions that can be useful in immediate prescribed burn planning.  However, machine learning (ML) models developed for studying fire systems predominantly focus only on wildfire modeling\cite{toulouse2017computer} using large-scale input data like historical weather conditions, topography, and fuel characteristics. Very few ML methods study prescribed fires \cite{cope2021using} - the majority of them focus on fire detection \cite{agastra2020evaluating}, burn severity \cite{perez2020evaluation}, and smoke management \cite{afrin2021machine}. However, for real-time prescribed fire planning, burn bosses require access to time-series forecasts of the prescribed fire evolution given initial environmental conditions - which is very different from modeling objectives that have been addressed in previous studies and will be the problem that we address in this paper. Furthermore, the lack of real-world input datasets for prescribed burns further exacerbates the problem \cite{gallagher2021reconstruction, linn2020quic}. This limits the usage of traditional ML models in scenarios where large-scale datasets are not available for training the model. 

% studying time-series evolution is very difficult compared to other modeling objectives
% prescribed-fires more difficult to model than wildfires

% wildfire emulators:
% 1. burned area prediction using initial conditions and CNN - different target
% 2. fireline prediction using initial conditions and PDEs - numeric instability, no evaluation on extrapolation (we build global model with different initial conditions)

Another major challenge is that conventional ML methods cannot accurately model the interaction of physical processes in a prescribed fire system (illustrated in Figure~\ref{fig:infographic}).  Integrating known physical constraints and domain knowledge in the model may reduce the need for large datasets and enable the ML model to learn physically consistent values \cite{willard2022integrating}. Such a physics-informed emulator would be extremely useful for planning fires and providing speedup over simulators in complex scenarios with heterogenous wind conditions, long time scales, or large land areas. Therefore, in our framework, we propose using physical constraints to regularize the loss function such that the model learns physically consistent fire spread behavior. Furthermore, the lack of observed datasets (due to prohibitive costs and ethical concerns) for prescribed burns further exacerbates the problem \cite{gallagher2021reconstruction, linn2020quic}. This limits the usage of traditional ML models in scenarios where large-scale datasets are not available for training the model. 
% We overcome this challenge by generating simulations from state-of-the-art simulator, QUIC-Fire, for estimating fuel density changes from prescribed burns. These simulations are used to learn an ML emulator for prescribed burn spread estimation.

% Another major challenge is that conventional ML methods cannot accurately model the interaction of physical processes in a prescribed fire system. Especially when building data-driven emulators or surrogate models for black-box-like fire simulators, we may not have access to intermediate variables and the physics modules used in the simulator. Therefore, integrating known physical constraints and domain knowledge in the model may reduce the need for large datasets and enable the model to learn physically consistent values using data-driven ML methods \cite{willard2022integrating}. A computationally efficient and physics-informed emulator would be extremely useful for planning fires in complex scenarios where there are multiple wind speeds, long time scales, or cover large land areas. Therefore, in our framework, we propose the use of physical constraints to regularize the loss function such that the model learns physically consistent fire spread behavior.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.25]{images/intro/Fuel_Cell.eps}
    \caption{\small QUIC-Fire fire mechanics \cite{linn2020quic}. The fuel moisture needs to dry up before the fire starts spreading in the cell. After the moisture dries up and other conditions are met for fire ignition, the fuel burns to completion. This fire behavior further changes as other factors start influencing the mechanics. }
    \label{fig:infographic}
\end{figure}


 
To overcome the above challenges, we propose using a physics-guided spatiotemporal model for predicting the fire spread behavior. To overcome the absence of real-world input data, we use QUIC-Fire simulations to learn the behavior of prescribed fires. The proposed emulator provides speedup over QUIC-Fire and can be used for faster than real-time prescribed fire forecasting. From initial wind conditions and user-provided ignition pattern (sequence map of how the burn bosses will ignite cells in a spatial grid), the emulator can provide the evolution of fire (in terms of fuel density, the mass of fire fuel per unit volume) over time.

% In addition to the initial parameter values used in QUIC-Fire, which are used as input to our emulator, we also utilize a source or reference fuel density distribution as input to the model. While our source/reference input data enables the model to learn the fire spread behavior, the input parameters from QUIC-Fire (initial wind speed, initial wind condition, and ignition pattern) help adapt the spread of the fire to different wind speeds and wind directions. We showcase our model's ability to generalize well to different wind conditions by integrating known physical constraints in our machine learning framework.


The summary of contributions of this work is provided next.

\begin{itemize}
    \item To the best of our knowledge, we propose the first physics-guided, prescribed fire emulator that can predict fuel density evolution from initial wind conditions and ignition patterns. 
    \item To overcome the challenges of limited input data, we enrich the feature set by including preexisting source domain data (fuel density similar in ignition pattern) as an additional channel. This ensures that the model overcomes the bias towards the overestimation of fuel and learns a more accurate fire spread behavior. 
    \item Using physics-guided learning, we incorporate physical constraints in the learning process to improve our generalization ability using limited input data while ensuring physical consistency in our predictions.
    \item Extensive experiments demonstrate the effectiveness of the proposed method in emulating prescribed fire behavior. The results of these experiments clearly demonstrate the superiority of our approach compared to other commonly used deep learning methods in terms of both prediction performance and physical consistency of the outputs.
\end{itemize}

In the proposed framework, we learn a model for estimating fuel density over time from initial wind conditions and ignition patterns. We include source domain fuel density sequence data as additional input to improve fire spread estimation. These source maps are preexisting data on fuel density evolution from a different wind scenario. To overcome the dearth of real data, we use simulations from QUIC-Fire, a computationally efficient prescribed fire simulator, as the ground truth for learning an ML emulator that can be useful in operational decision-making. We integrate physical knowledge into our framework to improve the generalization performance and the physical consistency of predicted fuel density. This physical knowledge is drawn from the assumptions and fire behavior that are encoded in the QUIC-Fire model. We also estimate fuel density and burned area as part of a graphical modeling structure that improves the representations learned for these quantities at different levels of abstraction. We evaluate the emulator's performance under varying wind conditions and ignition patterns. We demonstrate the efficacy of source domain data and physics-guided loss function, showing that our method can achieve good predictive performance. We have released our code in a temporary Google drive \href{https://drive.google.com/drive/folders/1kRRH_7an68mQGHUOcbilwupTdn5wyjhX?usp=sharing}{link}.



==> problemsetting0.tex <==

In this work, we study the evolution of fuel density caused by changing wind behavior and ignition pattern. Fuel density, the mass of fire fuel per unit volume, depletes as prescribed fire spreads and is commonly used to study the evolution of fires. We use $N$ simulation runs from the QUIC-Fire model as training examples to learn a data-driven emulator. As an emulator of the QUIC-Fire simulator, we observe the change in fuel density over a spatial region of $M \times P$ grid consisting of $M$ rows of cells and $P$ columns of cells. For each cell, we have dynamic inputs and static input variables, using the same initial conditions provided to QUIC-Fire as input. These scalar input parameter values are included as the static measurements in out training data. A QUIC-Fire user also provides an ignition pattern. This includes information on how different cells are ignited over time - these are the dynamic input parameters to QUIC-Fire, used to generate the fuel density time series. Ignition pattern is also used as a dynamic input to our model. Thus, at a time step in a training example, the input tensor can be represented as $\mathcal{X}_t \in \mathbb{R}^{M \times P \times C}$, where $C$ represents the number of input features provided to the model. And since each of our training examples are time-series with $n$ time steps, the input tensor with all $N$ training examples can be represented as $\mathcal{X} \in \mathbb{R}^{N \times n \times M \times P \times C}$.




A subset of input parameters $C-1$ are the input parameters of QUIC-Fire - initial wind speed, the initial wind direction, and the ignition pattern. In our data, we have five different ignition types, aerial (Fig~\ref{fig:aerial-observed}), outward (Fig~\ref{fig:outward-observed}), inward(Fig~\ref{fig:inward-observed}), strip north (Fig~\ref{fig:stripnorth-observed}) and strip south (Fig~\ref{fig:stripsouth-observed}) ignition patterns (Figure~\ref{fig:predictions}). 

% \begin{figure}[ht]
% \centering
% \begin{tabular}{cc}
% % \toprule
%  \subcaptionbox{\label{fig:intro-ignite-t0} Ignition at time step 20  \vspace{5pt} }{\includegraphics[scale=0.24]{images/intro/ignition-t0.png}} &
%   \subcaptionbox{\label{fig:intro-ignite-t1} Ignition at time step 49  \vspace{5pt} }{\includegraphics[scale=0.24]{images/intro/ignition-t1.png}}\\
% \subcaptionbox{\label{fig:intro-spread-t0} Fire Spread at time step 20  \vspace{5pt} }{\includegraphics[scale=0.24]{images/intro/spred-t0.png}} &
%  \subcaptionbox{\label{fig:intro-spread-t1} Fire Spread at time step 49  \vspace{5pt} }{\includegraphics[scale=0.24]{images/intro/spred-t1.png}}\\ 
% \end{tabular}
% \caption{Ignition versus fire spread. }
% \label{fig:intro}
% \vspace{-10pt}
% \end{figure}
\vspace{-10pt}
\begin{figure}[htp]
    \centering
    \includegraphics[scale=0.25]{images/intro/ignitedcells.png}
    \vspace{-10pt}
    \caption{Ignition versus fire spread}
    \label{fig:intro}
    \vspace{-10pt}
\end{figure}

\begin{figure}[h]
%\setlength{\belowcaptionskip}{-20pt}
    \centering
    \includegraphics[scale=0.4]{images/intro/data_split.png}
    \caption{Input source data setting. Source data includes fuel density for initial wind speed 1 m/s and 230$^\circ$ wind direction. Out-of-sample examples include target fuel densities with higher initial wind speed and wind direction }
    \label{fig:data_split}
    \vspace{-20pt}
\end{figure}


It is important to note that the ignition of cells is a precursor to the spread of fire. Figure~\ref{fig:intro} shows the difference between ignition and fire spread at two different time steps. As time increases, more cells are ignited, and other fuel and weather conditions lead to the spread of fire in nearby cells. While the ignition pattern is an important input that informs us about where the fire starts, it is insufficient to emulate the consequent spread of fire. % (rewrote this)Therefore for each ignition type, we provide a \textit{source} or \textit{reference} fuel density input that looks at the fire spread behavior. This source data differs for different training examples based on the ignition pattern. Depending on their ignition pattern, we select the fuel density time-series at initial wind speed 1 m/s and wind direction 230$^\circ$ as the source data for a training example. 
For each ignition type, we provide a source fuel density input to provide information about the fire spread behavior. Though the ignition pattern varies, the source data for model training always has an initial wind speed of 1 m/s and wind direction 230$^\circ$. 
We call this source data our \textit{standard source data setting}. In the experiments, we use the standard source data setting, unless otherwise stated. Visualizations of the standard source data are given in Appendix Figure~\ref{fig:refdata}. Figure~\ref{fig:data_split} describes the source data characteristics. Since we use the standard source data setting to extrapolate fuel density behavior to out-of-sample wind speed and wind directions in all our experiments(Fig.~\ref{fig:data_split}), we are able to evaluate the generalization power of our framework. For instance, to predict the fuel density for a prescribed burn with aerial ignition pattern at wind speed 7.5 and wind direction 300$^\circ$, we will use a source fuel density with aerial ignition, wind speed 1 m/s and wind direction 230$^\circ$. We holdout a set of five fuel density simulation runs for the five ignition types at wind speed 1 m/s and wind direction 230 $^\circ$ to use as source data for the training examples. We also extend our analysis to look at two other source data settings described in more detail in the Experiments section. Therefore, we use initial wind speed, initial wind condition, ignition pattern and source fuel density as input data and learn to predict fuel density $\mathcal{Y} \in \mathbb{R}^{N \times n \times M \times P \times 1}$. In our experiments, we train the model on input time-series from 0 to 50 seconds. During inference, we present results two sets of results. The primary results focus on the out-of-sample prediction performance for the model on test samples with wind conditions that are different from the source or reference input data wind conditions. Additionally, we also present the model performance in the extrapolation setting when predicting for 50 to 100 seconds using models trained on the first 50 seconds of the data.



The generalization of spatio-temporal models to extreme wind conditions is a challenging task. In addition, the variability in the spread of fire caused by the interaction of different inputs motivates the need to study different wind conditions. In our data, wind speed varies from slow winds at 1 m/s to faster winds at 15 m/s. Similarly, wind may blow from South-West (230$^\circ$) direction, going up to winds blowing from North-West (330$^\circ$). For instance, Figure~\ref{fig:model-diagram} includes reference data from strip north ignition type with the standard source data setting of wind speed 1 m/s and wind direction 230$^\circ$ while the target fuel density that we are trying to predict has different initial wind speed of 15 m/s and 330$^\circ$ initial wind direction. 

Moreover, fire also influences wind in the system by releasing energy and increasing the air temperature. While these initial ambient wind conditions affect fire behavior, the influence of fire on wind and its feedback on fuel density evolution is not well known due to limited input data. % is this accurate - is the influence of wind not well known? (Because it seems like the process based models do model the wind/fire movement) And is the issue limited input data? - ya it is not well known I read couple of papers. Will look for citations
We, therefore, have to utilize known physical constraints to overcome some of these challenges. We discuss this further in the next section. 

%the interaction of wind conditions with ignition patterns lead to different spreads of fire. For instance, igniting fire perpendicular to the wind leads to flank fires. Similarly, prescribed fires that are lit to burn against the wind direction are called back fires. Since they are burned against the wind direction, they have shorter flame lengths and burn more slowly. 
\begin{figure}[h]
    \centering
    % \includegraphics[width=0.30\textwidth]{images/intro/physics_guided_emulator.eps}
    \includegraphics[width=0.48\textwidth]{images/intro/model_updated.png}
    \vspace{-10pt}
    \caption{Physics-guided Emulator for fuel density estimation. Inputs include source fuel density, ignition pattern, initial wind speed, and initial wind direction.}
    \label{fig:model-diagram}
    \vspace{-10pt}
\end{figure}

==> relatedwork.tex <==

Traditional fire behavior simulator models \cite{finney1998farsite,linn2002studying, tymstra2010development, tolhurst2008phoenix, gaudreau2016borealfiresim}  have been used for simulating wildfires \cite{johnston2008efficient,sullivan2009wildland,gollner2015towards,katan2021abwise}. While these models have been adapted for generating prescribed fire simulations, they often make assumptions that may not be suitable for prescribed fire modeling and overlook the fire suppression behavior specific to prescribed fires. Additionally, their complex formulation and computational cost hinder their practical implementation for real-time operational decision-making \cite{schumaker2022hexfire, frangieh2018numerical}. Although QUIC-Fire \cite{linn2020quic} overcomes some of these challenges and offers faster runtime compared to other process-based models, it still has limitations in terms of real-time decision-making due to its computation time.


Machine learning (ML) models have emerged as computationally efficient alternatives to process-based models, demonstrating success in various wildfire modeling tasks, including fuel characterization, fire detection and mapping, fire weather, fire risk, and fire effect prediction \cite{jain2020review, zhang2022dynamic, zan2022emulation, bolt2022spatio}, long-term planning \cite{bao2015optimizing, mcgregor2016fast, penman2011bayes}, burned area prediction \cite{cortez2007data, safi2013prediction, storer2016pso, liang2019neural}, fire behavior prediction (e.g., fire spread, growth, severity) \cite{subramanian2017learning, chetehouna2015predicting,kozik2013adaptive}. However, methods developed for wildfire modeling may not generalize to prescribed fire modeling \cite{hiers2020prescribed, furman2018firetec, hoffman2018advancing, cope2021using,linn2020quic}. Wildfires are unplanned and may be caused by natural or accidental human ignitions. Prescribed fires are planned to meet management objectives and are ignited under pre-determined environmental conditions. In terms of fire mechanics, wildfires are often modeled as a single ignition point, eventually leading to an ellipsoid fire shape. In contrast, prescribed fires are ignited at several ignition points, often in terms of several fire lines. This creates a more complex interaction among the fire ignited at different points, leading to fire suppression. Prescribed fires are more complex and difficult to model compared to wildfires. Wildfire modeling often also looks at wildfires that have been burning for days, while prescribed fires are planned to be executed in a single day. Due to differences in time scales, wildfires are more heavily impacted by moisture content in the atmosphere and weather patterns over several days, while the effect of these exogenous variables may not be that prominent for prescribed fires. This leads to a difference in fire behavior in a wildfire and a prescribed fire \cite{hiers2020prescribed, hoffman2018advancing,furman2018firetec}. 

Advancements in physics-guided ML have also contributed to wildfire modeling \cite{allaire2021emulation, bottero2020physics}. However, the physical assumptions made by current methods are not suitable for prescribed fire modeling, and these emulators may address different modeling problems unrelated to prescribed fire. These methods overlook the interaction of fire with ambient wind conditions and may suffer from numerical instability \cite{bottero2020physics}. In contrast, our framework leverages simulations from QUIC-Fire as ground truth, enabling the learning of the two-way interaction between environmental conditions and fire behavior without making strong assumptions. Moreover, previous studies in prescribed fire modeling have not extensively explored the specific problem of prescribed fire evolution modeling based on initial environmental conditions \cite{cope2021using, agastra2020evaluating, afrin2021machine, perez2020evaluation}. This capability is crucial for effective prescribed fire planning. By addressing this gap, our framework fills an important need in the existing ML literature. Integrating physical knowledge has been used in several domain adaptations and transfer learning problems in computer vision \cite{lengyel2021zero, luo2022physics, xu2021phymdan, ozdaugli2022physics}. Similarly, our framework overcomes the challenge of limited target domain input data by learning from the source domain dataset. 


% Machine learning methods have been developed for studying other prescribed fire modeling problems such as fire detection \cite{agastra2020evaluating}, burn severity prediction\cite{perez2020evaluation}, burned area prediction \cite{cope2021using}, and smoke management \cite{afrin2021machine}. In contrast to previous studies, our paper aims to address the specific problem of providing burn bosses with real-time time-series forecasts of prescribed fire evolution based on initial environmental conditions, which is crucial for effective prescribed fire planning but has not been extensively explored in the existing ML literature.




% To study fire spread and behavior, these previously proposed methods look at input features relating to ignition factors, fuel conditions, and climate factors which can come from historical survey data, process-based models, or satellite imagery data \cite{zhu2022building, pimont2021prediction}. In contrast, our framework only has access to initial wind conditions and ignition patterns which are used to emulate the fuel density sequence over a spatial grid. %could mention the use of the reference dataset here
% Furthermore, many of the previous studies that utilize domain knowledge in wildfire modeling are limited to the use of genetic algorithms to optimize input parameters of empirical fire simulators \cite{sample2016spatially, artes2017time, denham2012dynamic, rodriguez2008adaptive}. Again, this requires significant computation time to generate fire spread metrics \cite{jain2020review, schumaker2022hexfire}.
% Recent deep learning-based emulators \cite{cope2021using,allaire2021emulation} also use simulation input as features, similar to our model. However, these reports also utilize more informative ``positional" inputs and additional fuel parameters to model the fire spread. These studies are also limited by their applicability to non-dynamic datasets since they utilize CNN models. Modern fire management practices include prescribed fires that aid in fire preparedness. Predicting the behavior and evolution of prescribed fires is essential for the management of vegetation, fire suppression, and prevention of wildfires. While a recent study proposed models for prescribed fires \cite{cope2021using}, they also use the output of the QUIC-Fire model for training the model, limiting its applicability in use cases that cannot run simulations for generating training data due to computational and time constraints.



% Similar to these methods, we overcome the challenges of limited target domain input data by learning from the source domain dataset. In our framework, the source and target domains are fuel density data that are similar in their ignition patterns used for lighting the prescribed fires. However, the environmental conditions, including wind speed and direction, may be different.

%In our experiments, we also investigate how learning these statistical similarities using Gram-based representations of source and target fuel densities can help enable improved prescribed fire emulation.

By incorporating not only the change in fuel density over time but also fire spread metrics in the loss function, our framework provides a comprehensive solution for predicting and monitoring prescribed fire behavior. Overall, our framework offers a unique and powerful method that addresses the complexities of emulating prescribed fire evolution. It integrates physical constraints, leverages domain knowledge, and provides fast time-series forecasts, making it a valuable tool for burn bosses and stakeholders involved in prescribed fire planning and decision-making.

% The model presented in this work is unique in that it provides a powerful framework for emulating spatial and temporal prescribed fire evolution. This framework enables the integration of physical constraints and domain knowledge, allowing for reductions in data needs. In addition, for burn bosses and public stakeholders, understanding the general direction of the spread of fire is important for making operational decisions. For this, predicting and monitoring evolution in fire metrics like rate of spread and burned area index is also imperative. Therefore, in addition to predicting the change in fuel density over time, we also incorporate the rate of spread and burned area in our loss metrics. These attributes of the framework aid in the development of fire prediction models that are data-efficient and generalizable.




==> results0.tex <==
\subsection{Experimental Setup}



\subsubsection{Baselines}

Models like CNN and UNet are commonly in prescribed fire and wildfire modeling literature. Therefore, we compare ConvLSTM based model defined in the methods section with CNN and Unet-based baseline methods for fuel density prediction.

\paragraph{\textbf{CNN}} CNN has been used as an emulator for the QUIC-Fire model \cite{cope2021using}. As a segmentation model, the CNN model was the first to be able to predict burned and unburned regions with significant reduction in computational time over QUIC-Fire. Since we are also interested in studying the change in fuel density due to the spread of fire, we use a regression CNN model in our experiments. We stack eleven sets of convolution operations with ReLU activation and kernel of size three and max pooling of size two after every two convolution layers. While the previous CNN emulator predicted the fire spread frame 50 time steps ahead, we emulate the whole fire spread time series.

\paragraph{\textbf{UNet}} UNets are powerful spatio-temporal models used in a wide range of applications. We include BCDU-Net as one of the baselines \cite{azad2019bi}. This U-Net includes Bi-directional ConvLSTM layers and reuses feature maps for precise segmentation in multiple different types of medical imaging datasets. In the encoding path of the model, a learned feature map at each stage is concatenated with feature maps of the current layer. Through these densely connected convolutions, the network learns more diverse feature representations. The decoding path performs upsampling and utilizes bi-directional ConvLSTM layers. As opposed to the original BCDU-Net implementation which was a segmentation model used on medical images, we build a regression model for fuel density prediction.


\begin{table}[h]
    \centering
    \scriptsize
    
    \begin{tabular}{p{2cm}llllll}
        \hline

         & QUIC-Fire &  PGCL & CL & CNN & UNET \\ \cmidrule(lr){1-6}
        Minimum & 55 & 11 & 48 & 24 & 32 \\
        Mean & 83 & 25 & 51 & 26 & 34 \\
        Maximum & 232 & 40 & 54 & 31 & 38 \\
        \hline

    \end{tabular}
    
    \caption{\small Model Inference Time}
    \label{tab:inference-time}
    \vspace{-20pt}
\end{table}


\textbf{Datasets:} We use simulation runs from the QUIC-Fire model to learn the prescribed fire emulator. We simulate and use 100 runs as training examples. The simulation runs are for an idealized grassland setting with two-dimensional evolution of fires captured in 300 x 300 cells grid over $n$ time steps at 1 second time intervals. As mentioned in the previous section, the simulation runs consist of 5 different ignition patterns, 7 wind speeds and 11 different wind directions. To build the physics-guided model the experimental setting use data with $n=$50, $N=$100, $M=P=$300 and $C=$4.

\textbf{Experiments Details:} We randomly split the 100 simulation runs and place 50\% of the data into training and rest into test data with each comprising of 50 samples (train and test set statistics given in Appendix). Therefore, each of the datasets have features with dimensionality $50 \text{ simulation runs } \times 50 \text{ time steps }\times 300 \text{ rows } \times 300 \text{ rows } \times 4 \text{ features }$. With batch size 1 and using the Adam optimization method for gradient estimation, we train each of the models for 250 epochs. Learning rate, number of layers and hidden units are fine-tuned using random grid search in the CNN and ConvLSTM models. The architecture for UNet is derived from the BCDU-Net framework with learning rate fine-tuned using random grid search. In our experiments, we use $\epsilon=$ 0.001 for the physical constraint loss masking. We also use $\epsilon_b=$0.1 and $\epsilon_u=$0.65 for the burned and unburned loss masking, respectively.

\textbf{Metrics:} To accurately study the performance of our ML models, we evaluate several metrics that compute how well the model predicts the evolution of fire over time. In the tables, downward arrow indicated that lower values of evaluation metric indicate better model performance.

\noindent \textbf{Physics guided loss terms:} The physics guided loss terms described in the methods section can also be computed for evaluating the model's performance in accurately capturing different physical constraints. We therefore evaluate MSE, burned area MSE, unburned area MSE and fire metric MSE (ROS MSE + BA MSE) .

\noindent \textbf{Dynamic MSE (DMSE):} We formulate a metric that evaluates model performance based on change in fuel density over time. For time steps with bigger change in the observed fuel density, we ensure that the error in predictions are penalized more,

% \begin{equation*}
%     V_{t, t-1} = (||\hat{M}_t - M_t|| - ||\hat{M}_ {t-1} - M_{t-1}||)
% \end{equation*}

% \begin{equation}
% \begin{split}
%     VMAE & = \frac{\sum_M (1-\Delta(M_t - M_{t-1})\Delta(\hat{M}_t -  \hat{M}_{t-1})) \cdot V_{t, t-1}
%     }{ \sum_M (1-\Delta(M_t - M_{t-1})\Delta(\hat{M}_t -  \hat{M}_{t-1}))}
% \end{split}    
% \end{equation}

\begin{equation}
\begin{split}
    DMSE & = \frac{\sum_N (\Delta(Y_t - Y_{t-1})) \cdot (||\hat{Y}_t - Y_t||)
    }{ \sum_N (\Delta(Y_t - Y_{t-1}))}.
\end{split}    
\end{equation}

We can further validate the physical consistency of the predictions by evaluating how often the physical constraints are met in the predicted values using the following metrics.
\noindent \textbf{Metric}$_{\text{PC}}$ is the percentage of cells that follow the physical constraint in the predicted time-series. \textbf{Metric}$_{\text{Burned}}$ is the percentage of unburned cells that are predicted to be burned. \textbf{Metric}$_{\text{Unburned}}$ is the percentage of unburned cells where fuel densities are underestimated. \textbf{Metric}$_{\text{False Positive}}$ is the percentage of burning cells that are predicted to be burned. \textbf{Metric}$_{\text{False Negative}}$ is the percentage of burning cells that are predicted to be unburned.


% In our experiments, we also show that learning statistical similarities between the reference and target fuel density data enables learning of better physical properties compared to a MSE based loss function. We compare the density distribution of fuel density among the physics-based model, Gram loss-based model and the MSE only model.

% \noindent \textbf{MMD:} Domain adaptation and transfer learning methods focus on minimizing the distribution discrepancy between the source and target domains \cite{jing2019neural}. In computer vision, this facilitates matching of feature distribution between the two domains and enabling improved model performance in the target domain. We utilize Maximum Mean Discrepancy (MMD) as an evaluation metric to analyze if we see similar difference in the predicted distribution of different domains (wind conditions and ignition patterns) as we see in the observed distribution of fuel density. We compute pairwise MMD between different test samples to evaluate the similarity between observed and predicted fuel density distribution.


\begin{figure*}[!h]
\captionsetup[subfigure]{labelformat=empty,skip=-5pt}

\centering
\renewcommand{\arraystretch}{0.5}
\begin{tabular}{m{1.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}m{2.5cm}}
 % &&& \subcaptionbox{\includegraphics[scale=0.30]{images/colorbar.png}}&& \\
% \multicolumn{6}{c}{
% \subcaptionbox{\includegraphics[scale=0.40]{images/colorbar.png}}
% }  
%  \\ 
% \toprule

\centering
 s=1, d=280, ip=Inward & \subcaptionbox{\label{fig:inward-observed} Observed  }{\includegraphics[scale=0.20]{images/individual/obs/pred-17.eps}} &
 \subcaptionbox{\label{fig:inward-all}Physics-Guided  }{\includegraphics[scale=0.20]{images/individual/all/pred-17.eps}} &
 \subcaptionbox{\label{fig:inward-mse} MSE Only  }{\includegraphics[scale=0.20]{images/individual/mse/pred-17.eps}} &
 \subcaptionbox{\label{fig:inward-cnn} CNN  }{\includegraphics[scale=0.20]{images/individual/cnn/pred-17.eps}} &
 \subcaptionbox{\label{fig:inward-unet} UNet  }{\includegraphics[scale=0.20]{images/individual/unet/pred-17.eps}} \\ 


\centering
 s=2, d=320, ip=Strip South & \subcaptionbox{\label{fig:stripsouth-observed}  Observed  }{\includegraphics[scale=0.20]{images/individual/obs/pred-38.eps}} &
 \subcaptionbox{\label{fig:stripsouth-all}Physics-Guided  }{\includegraphics[scale=0.20]{images/individual/all/pred-38.eps}} &
 \subcaptionbox{\label{fig:stripsouth-mse} MSE Only  }{\includegraphics[scale=0.20]{images/individual/mse/pred-38.eps}} &
 \subcaptionbox{\label{fig:stripsouth-cnn} CNN  }{\includegraphics[scale=0.20]{images/individual/cnn/pred-38.eps}} &
 \subcaptionbox{\label{fig:stripsouth-unet} UNet  }{\includegraphics[scale=0.20]{images/individual/unet/pred-38.eps}} \\ 


\centering
 s=3, d=310, ip=Strip North  & \subcaptionbox{\label{fig:stripnorth-observed}Observed  }{\includegraphics[scale=0.20]{images/individual/obs/pred-43.eps}} &
 \subcaptionbox{\label{fig:stripnorth-all} Physics-Guided  }{\includegraphics[scale=0.20]{images/individual/all/pred-43.eps}} &
 \subcaptionbox{\label{fig:stripnorth-mse} MSE Only  }{\includegraphics[scale=0.20]{images/individual/mse/pred-43.eps}} &
 \subcaptionbox{\label{fig:stripnorth-cnn} CNN  }{\includegraphics[scale=0.20]{images/individual/cnn/pred-43.eps}} &
 \subcaptionbox{\label{fig:stripnorth-unet} UNet  }{\includegraphics[scale=0.20]{images/individual/unet/pred-43.eps}} \\ 


\centering
 s=7.5, d=300, ip=Outward & \subcaptionbox{\label{fig:outward-observed}  Observed }{\includegraphics[scale=0.20]{images/individual/obs/pred-27.eps}} &
 \subcaptionbox{\label{fig:outward-all} Physics-Guided }{\includegraphics[scale=0.20]{images/individual/all/pred-27.eps}} &
 \subcaptionbox{\label{fig:outward-mse}  MSE Only  }{\includegraphics[scale=0.20]{images/individual/mse/pred-27.eps}} &
 \subcaptionbox{\label{fig:outward-cnn}  CNN  }{\includegraphics[scale=0.20]{images/individual/cnn/pred-27.eps}} &
 \subcaptionbox{\label{fig:outward-unet}  UNet }{\includegraphics[scale=0.20]{images/individual/unet/pred-27.eps}} \\



\centering
%\captionsetup{skip=1pt}
s=15, d=270, ip=Aerial & \subcaptionbox{\label{fig:aerial-observed} Observed  }{\includegraphics[scale=0.20]{images/individual/obs/pred-44.eps}}  &
 \subcaptionbox{\label{fig:aerial-all} Physics-Guided   }{\includegraphics[scale=0.20]{images/individual/all/pred-44.eps}} &
 \subcaptionbox{\label{fig:aerial-mse} MSE Only  }{\includegraphics[scale=0.20]{images/individual/mse/pred-44.eps}} &
 \subcaptionbox{\label{fig:aerial-cnn} CNN  }{\includegraphics[scale=0.20]{images/individual/cnn/pred-44.eps}} &
 \subcaptionbox{\label{fig:aerial-unet} UNet  }{\includegraphics[scale=0.20]{images/individual/cnn/pred-44.eps}} \\ 
 \centering
 &&&& \subcaptionbox{\includegraphics[scale=0.40]{images/colorbar.png}}& \\
\end{tabular}
\caption{\small \textbf{Individual Predictions}: The values in the first column are the test sample's wind speed (m/s), s,  wind direction ($^\circ$), d, and ignition type, ip. We show the 50$^{th}$ second prediction to compare the model performance. Physics-Guided and MSE Only are ConvLSTM models. Legend for fuel density values given on the bottom right corner.}
\label{fig:predictions}
\vspace{-10pt}
\end{figure*}

\subsection{Results and Discussion}


\subsubsection{Reference Input Data:}

Reference or source fuel density enables the model to learn spatio-temporal changes in target fuel density. Table~\ref{tab:baselines} shows a comparison of CNN, UNet and ConvLSTM models in learning fire behavior in the absence and presence of source fuel density input data. As described in the problem setting, we use the standard source data setting. The MSE values reflect that by including the source fuel density sequence data as one of the features, we are able to improve the emulation of the prescribed burns. Moreover, ConvLSTM is able to perform better than the CNN and UNet based models in predicting fuel density distribution. For further experiments, we explore ConvLSTM based spatio-temporal model for physics-guided learning.



% \begin{figure}[h]
% \centering
% \begin{tabular}{m{8cm}}
% % \toprule
% \centering
%  \subcaptionbox{1, 280, Inward}{\includegraphics[scale=0.2]{images/appendix/ws/ws-17.eps}} \\ 
 
%  \subcaptionbox{7.5, 300, Outward}{\includegraphics[scale=0.2]{images/appendix/ws/ws-27.eps}} \\ 
 
%  \subcaptionbox{15, 270, Aerial}{\includegraphics[scale=0.2]{images/appendix/ws/ws-44.eps}} \\ 
 
%  \subcaptionbox{3, 310, Strip North}{\includegraphics[scale=0.2]{images/appendix/ws/ws-43.eps}} \\ 
 
 
%  \subcaptionbox{2, 320, Strip South}{\includegraphics[scale=0.2]{images/appendix/ws/ws-38.eps}} \\ 

% \end{tabular}
% \caption{\textbf{Individual Predictions}: Predicting at 100 seconds with different wind speed and wind direction reference fuel density input. From left to right, first column: wind speed 1 and wind direction 230, second column: wind speed 7.5 and wind direction 280, third column: observed fuel density   }
% \label{fig:reference-ws-extrapolate}
% \vspace{-10pt}
% \end{figure}





\begin{table}[h]
    \centering
    \large
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{p{2cm}llllll}
        \hline
      
        Method & MSE ($\downarrow$) & Burned & Unburned  & Fire Metrics  & DMSE($\downarrow$) \\
         && MSE($\downarrow$)& MSE($\downarrow$)& MSE($\downarrow$)&\\\cmidrule(lr){1-6}
        CNN (w/o reference)     & 1.4e-1     & 1.4e-1 & 2.8e-1 & 1.4e-1 & 2.6e-3  \\
        U-Net (w/o reference)    & 1.2e-1     & 2.0e-1 & 1.2e-1 & 1.3e-2 & 3.3e-3  \\
        ConvLSTM (w/o reference)  & 2.7e-3 & 2.7e-3 & 5.5e-3 & 2.7e-1 & 9.3e-3 \\
        CNN     & 2.0e-4    & 2.0e-4 & 4.3e-3 & 2.2e-2 & 3.0e-4  \\
        U-Net     & 5.3e-3    & 3.1e-4  & 5.3e-3 & \textbf{1.3e-3} & 1.7e-3\\
        ConvLSTM  & \textbf{1.2e-8}    & \textbf{1.2e-8} & \textbf{2.5e-8} & 1.4e-3 & \textbf{1.2e-3} \\

        \hline
    \end{tabular}
    }
    \caption{\small Test set model performance up to 50 seconds. ConvLSTM with reference input data (standard source data setting) outperforms other methods.}
    \label{tab:baselines}
    \vspace{-25pt}
\end{table}




\subsubsection{Adding Physics}
\begin{table*}[ht]
    \centering
    \small
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccccccc}
        \toprule
        \multirow{1}{*}{\bfseries  } & 
        % \multicolumn{3}{c}{\bfseries Attributes } & 
        \multicolumn{5}{c}{\bfseries Physics-Guided - Metric} & 
        \multicolumn{5}{c}{\bfseries MSE Only - Metric}\\ 
        % \cmidrule(lr){2-4}
        \cmidrule(lr){2-6}
        \cmidrule(lr){7-11}
         Sample & PC (\downarrow) & Burned (\downarrow)& Unburned (\downarrow)& \begin{tabular}{@{}c@{}}False \\ Positive (\downarrow)\end{tabular} & \begin{tabular}{@{}c@{}}False \\ Negative (\downarrow)\end{tabular}& PC (\downarrow) & Burned (\downarrow)& Unburned (\downarrow)& \begin{tabular}{@{}c@{}}False \\ Positive (\downarrow)\end{tabular} & \begin{tabular}{@{}c@{}}False \\ Negative (\downarrow)\end{tabular} \\
         \midrule
         Row 1: s=1, d=280, inward  & 0.01 & 0.00 & 1.46 & 0.00 & 11.73 & 0.01 & 0.34 & 1.42 & 0.33 & 76.44 \\
         Row 2:, s=2, d=320, strip south  & 0.00 & 0.01 & 1.60 & 0.01 & 37.73 & 0.13 & 0.35 & 86.40 & 0.37 & 47.82 \\
         Row 3: s=3, d=310, strip north  & 0.01 & 0.06 & 1.79 & 0.09 & 38.55& 0.06 & 0.36 & 3.58 & 0.39 & 31.39\\
         Row 4: s=7.5, d=300, outward  & 0.00 & 0.05 & 0.71 & 0.12 & 18.67 & 0.05 & 0.36 & 2.75 & 0.49 & 20.05 \\
         Row 5: s=15, d=270, aerial  & 0.01 & 0.34 & 1.84 & 0.42 & 38.53& 0.21 & 92.12 & 92.91 & 91.74 & 94.75\\

         \bottomrule
    \end{tabular}
    }
    \caption{\small Physical consistency evaluations metric for test samples displayed in Figure~\ref{fig:predictions}. s=wind speed, d= wind direction. }
    \label{tab:pred_label}
    \vspace{-15pt}
\end{table*}

\begin{table}
    \centering
    \scriptsize
    \begin{tabular}{p{2cm}llllll}
        \hline
        % \multirow{2}{*}{\bfseries  } & 
        % \multicolumn{5}{c}{\bfseries Idealized Grasslands / Ignition Pattern - Wise}  
        %  \\ 
        % \cmidrule(lr){2-6}
        % \cmidrule(lr){7-11}

        Method & MSE ($\downarrow$)& Burned & Unburned & Fire Metrics & DMSE ($\downarrow$)\\
        && MSE ($\downarrow$)& MSE ($\downarrow$) & MSE ($\downarrow$) & \\
        \cmidrule(lr){1-6}

        ConvLSTM (MSE)  & 1.2e-8    & 1.2e-8 & 2.5e-8 & 1.4e-2 & 1.7e-3 \\
        % ConvLSTM (MSE+Gram matrix loss) & 2.3e-5 & 2.3e-5 & 1.7e-5 & 2.0e-4 & 1.6e-5 \\
        ConvLSTM (MSE+Burned) & 4.8e-3     & 4.8e-3 & 9.7e-3 & 4.9e-3 & 1.1e-2  \\
        ConvLSTM (MSE+Unburned) & 2.3e-4     & 2.3e-4 & 4.6e-4 & 5.6e-4& 4.0e-3 \\
        ConvLSTM (MSE+Physical Constraint) & 9.3e-6     & 9.3e-6 & 1.8e-5 & 1.8e-4& 4.8e-3 \\
        ConvLSTM (MSE+Fire Metrics) & 2.0e-5     & 2.0e-5 & 4.1e-5 & 1.1e-4 & 7.4e-5\\
%        ConvLSTM (Physics-Guided + Gram matrix Loss)     & 2.8e-9    & 2.8e-9 & 5.7e-10 & 3.1e-4 & 8.5e-7  \\
        ConvLSTM (Physics-Guided) & \bf{3.2e-13} & \bf{3.2e-13} & \bf{4.7e-12} & 4.9e-6& 4.6e-8  \\ 
        \cdashline{1-6}
        ConvLSTM (Physics-Guided, reference wind speed 7.5, wind direction 280) & 6.5e-10 & 6.5e-10 & 1.3e-9 & \bf{7.5e-10} & \bf{2.6e-10} \\
         
        ConvLSTM (Physics-Guided, reference wind speed 15, wind direction 330)  & 2.6e-8 & 2.6e-8 & 5.3e-8 & 2.6e-9 & 3.0e-10\\ 
        
        \hline
       
    \end{tabular}
    \caption{\small Test set model performance for models trained upto 50 seconds. ConvLSTM with all physics-guided loss terms outperforms other methods. Physics-Guided refers to MSE +Burned +Unburned +Physical Constraint +Fire Metrics.}
    \label{tab:losses}
    \vspace{-20pt}
\end{table}

\begin{figure*}[ht]
\centering
\begin{tabular}{m{3.1cm}m{3.1cm}m{3.1cm}m{3.1cm}m{3.1cm}}
% \toprule
\centering
 \subcaptionbox{1, 280, Inward}{\includegraphics[scale=0.2]{images/mseovertime/pred-17.eps}} &
 
 \subcaptionbox{2, 320, Strip South}{\includegraphics[scale=0.2]{images/mseovertime/pred-38.eps}} &
 
 
 \subcaptionbox{3, 310, Strip North}{\includegraphics[scale=0.2]{images/mseovertime/pred-43.eps}} &

  \subcaptionbox{7.5, 300, Outward}{\includegraphics[scale=0.2]{images/mseovertime/pred-27.eps}} &
 
 \subcaptionbox{15, 270, Aerial}{\includegraphics[scale=0.2]{images/mseovertime/pred-44.eps}} 
\\ 

\end{tabular}
\caption{\small \textbf{Individual Predictions}: Extrapolation behavior beyond 50 time steps.  }
\label{fig:msebytime-comparison}
\vspace{-10pt}
\end{figure*}








We investigate the effect of different physical constraints on prescribed fire emulation. The model performance in terms of the test set evaluation metrics is given in Table~\ref{tab:losses}. While adding the individual constraints help improve the model over the standard spatio-temporal models, we are able to achieve the best model performance using the "Physics-Guided", physics-guided model. This model utilizes the loss function $\mathcal{L_P} = \mathcal{L_{MSE}}+\mathcal{L_{PC}}+\mathcal{L_{\text{Burned}}}+\mathcal{L_{\text{Unburned}}}+\mathcal{L_{ROS}}+\mathcal{L_{BA}}$. This physics-guided model outperforms other ConvLSTM variants. As shown by the DMSE metric, the physics-guided model shows improvement in prediction skill for frames that corresponded with rapidly changing fuel density values.  Several of the ConvLSTM variants also show a reduction in fire metric MSE values suggesting that overall rate of spread and burned area percentage in predictions closely emulated the observed fuel density. %We also experiment adding the Gram matrix loss in the "Physics-Guided" physics-guided loss function ($\mathcal{L} = \mathcal{L_{P}}+\mathcal{L_{G}}$). This provides improvement in the fire metrics loss and DMSE when compared to the ConvLSTM model with loss $\mathcal{L} = \mathcal{L_{MSE}}+\mathcal{L_{G}}$.

While the MSE values are useful to evaluate the average model performance, investigating individual prediction examples can be useful to ensure generalization under different distributional settings. Figure~\ref{fig:predictions} shows the individual predictions at the 50$^{\text{th}}$ second and also outlines the test sample attributes for comparison. We compare the ConvLSTM model MSE loss function with MSE loss function and ConvLSTM physics-guided model ($\mathcal{L_P}$) with the CNN (MSE loss function) and UNet (MSE loss function) models. We notice that the physics-guided model has the most stable predictions while other methods are over-burning unburned cells and under-burning burned areas. This behavior is evident in extreme wind conditions, particularly higher wind speeds and wind direction originating from 330$^\circ$. We see that baseline models in the last row (wind speed of 15 m/s) have difficulty in predicting the unburned area. The ConvLSTM MSE only model is able to predict well for lower wind speeds compared to other baselines that are over-estimating fuel density in the burned area. In models that are not informed by physical constraints in the loss term, we also notice higher fuel density predictions in cells surrounding the fire perimeter. This behavior arises due to complex wind dynamics in that region. In absence of physics guidance, the standard ML models are inaccurately predicting fuel density in that region. Furthermore, in the cells that are predicted to be burned, the physics-guided model is able to predict the lower fuel density values accurately. Among the models, the physics-guided model is able to achieve the most accurate predictions for fuel density values.

We can further compare the model performance in their ability to accurately capture the physical behavior of the fire spread. Results in Table~\ref{tab:pred_label} summarize some physical behavior metrics for test samples presented in Figure~\ref{fig:predictions}. The results suggest that the physics-guided model (Physics-Guided) is able to achieve more physical consistency in the predictions. The physics-guided model has a lower proportion of cells where the physical constraint is not met. The physics-guided model also has a lower proportion of falsely predicted burned cells and falsely predicted unburned cells. This is also evident in the visualizations of the individual predictions. The physics-guided model provides better burn predictions than the standard ConvLSTM model as shown in the lower values for the physical consistency evaluation metrics in Table~\ref{tab:pred_label}. 






\subsubsection{Changing Reference Data}




% \begin{figure}[t!]
% \captionsetup[subfigure]{skip=-5pt}
% \centering

% \begin{tabular}{m{8cm}}
% % \toprule
% %\centering
%  \subcaptionbox{1, 280, Inward}{\includegraphics[scale=0.2]{images/refws/pred-17.eps}} \\ 

%  \subcaptionbox{2, 320, Strip South}{\includegraphics[scale=0.2]{images/refws/pred-38.eps}} \\ 

%  \subcaptionbox{3, 310, Strip North}{\includegraphics[scale=0.2]{images/refws/pred-43.eps}} \\ 

%  \subcaptionbox{7.5, 300, Outward}{\includegraphics[scale=0.2]{images/refws/pred-27.eps}} \\ 
 
%  \subcaptionbox{15, 270, Aerial}{\includegraphics[scale=0.2]{images/refws/pred-44.eps}} \\  

% \end{tabular}

% \caption{\small\textbf{Individual Predictions}: Predicting with different wind speed and wind direction reference fuel density input. From left to right, first column: wind speed 1 and wind direction 230, second column: wind speed 7.5 and wind direction 280, third column: wind speed 15 and wind direction 330, fourth column: observed fuel density   }
% \label{fig:reference-ws}
% \vspace{-10pt}
% \end{figure}

Since the source fuel density has a big impact on the model performance, we can also investigate using source input data with different wind characterizations. We build two additional physics-guided models - with average wind conditions and with extreme wind conditions. Average wind conditions are those with wind speed of 7.5 m/s and wind originating from wind direction 280$^\circ$. The extreme wind conditions refer to wind speed 15 m/s and wind direction 330$^\circ$. The results for these models compared with the standard source data setting of 1 m/s and 230$^\circ$ are given in Table~\ref{tab:losses} and Figure~\ref{fig:reference-ws}. In terms of the evaluation metrics, the average wind condition source data provides better fire metric MSE and DMSE values. For other metrics, the standard source data is able to provide the best model performance. Figure~\ref{fig:reference-ws} shows that the models under the average source data setting and the extreme source data setting underestimate fuel in unburned cells. This is even more conspicuous in the extreme source data setting in test runs for higher wind speed and wind direction conditions. The results indicate that using the standard source data setting enables us to learn fire spread behavior under stable wind conditions. For more extreme wind conditions, the fire mechanics are more chaotic and uncertain. This makes learning from extreme source data setting more difficult and therefore leads to higher prediction error. The average source setting is another alternative that can be explored further in the future work. More results comparing the different source settings is given in Appendix, Figure~\ref{fig:reference-ws-extrapolate}.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{images/refws/ws.eps}
    \caption{\small \textbf{Individual Predictions}: Predicting with different input source data settings. s=speed, d=direction.}
    \label{fig:reference-ws}
\end{figure}

% \begin{table}[h]
%     \centering
%     \scriptsize
    
%     \begin{tabular}{p{2cm}llllll}
%         \hline
%         % \multirow{2}{*}{\bfseries  } & 
%         % \multicolumn{5}{c}{\bfseries Idealized Grasslands / Ignition Pattern - Wise}  
%         %  \\ 
%         % \cmidrule(lr){2-6}
%         % \cmidrule(lr){7-11}

%         Method & MSE ($\downarrow$)& Burned & Unburned & Fire Metrics & DMSE ($\downarrow$)\\
%         && MSE ($\downarrow$)& MSE ($\downarrow$) & MSE ($\downarrow$) & \\ \cmidrule(lr){1-6}
%         ConvLSTM (MSE)  & 2.2845   & 3.6972 & 5.3480 & 2.7404 & 0.0014 \\
% %        ConvLSTM (MSE+gram matrix loss) & 0.0114   & 0.0096 & 0.0192 & 0.0105 & 0.0004  \\
%         ConvLSTM (MSE+Burned)   & 0.0080   & \textbf{0.0063} & 0.0127 & 0.0069 & 0.0004   \\
%         ConvLSTM (MSE+Unburned) & 0.0258   & 0.0236 & 0.0472 & 0.0246 & 0.0006 \\
%         ConvLSTM (MSE+Physical Constraint) & 0.0101   & 0.0079 & 0.0158 & 0.0082 & 0.0006  \\
%         ConvLSTM (MSE+Fire Metrics) & 0.0097   & 0.0080 & 0.0161 & 0.0086 & 0.0003\\
%         ConvLSTM (MSE + Physics-Guided) & \textbf{0.0017}   & 0.0223 & \textbf{0.0030} & \textbf{0.0017} & \textbf{0.0001}   \\
%         \hline
%         \hline
%     \end{tabular}
    
%     \caption{\small Test set model performance for models trained on 50 seconds to time steps beyond 50 seconds. ConvLSTM with all physics-guided loss terms outperforms other methods.}
%     \label{tab:losses-ood}
%     \vspace{-20pt}
% \end{table}


% \subsubsection{Extrapolation in Time}


\begin{figure}
\centering
\begin{tabular}{cc}
% \toprule
 \subcaptionbox{\label{fig:msebywind-alllosses} Physics-Guided, 50$^{\text{th}}$ time step   }{\includegraphics[scale=0.28]{images/msebywind/alllosses_msebywind_insample.eps}} &
 \subcaptionbox{\label{fig:msebywind-mseonly} MSE only loss, 50$^{\text{th}}$ time step   }{\includegraphics[scale=0.28]{images/msebywind/mseonly_msebywind_insample.eps}} \\
 \subcaptionbox{\label{fig:ROSmsebywind-alllosses} Physics-Guided, 100$^{\text{th}}$ time step   }{\includegraphics[scale=0.28]{images/msebywind/alllosses_msebywind_extrapolate.eps}} &
 \subcaptionbox{\label{fig:ROSmsebywind-mseonly} MSE only loss, 100$^{\text{th}}$ time step   }{\includegraphics[scale=0.28]{images/msebywind/mseonly_msebywind_extrapolate.eps}} \\ 
\end{tabular}
\caption{MSE by wind conditions for ConvLSTM models with different loss functions. Color represents the MSE values.}
\label{fig:msebywind}
\vspace{-15pt}
\end{figure}

% We can investigate the prediction distribution for time steps beyond 50 seconds. We therefore test the extrapolation model performance from 50 to 100 seconds. Table~\ref{tab:losses-ood} summarises the average model performance. The physics-guided model is able to outperform other methods. The evolution of MSE at each time step can also be investigated. Figure~\ref{fig:msebytime-comparison} provides examples of MSE evolution for different test samples. For all time steps upto 50 seconds, we see lower MSE values for the physics-guided model. In the test samples with strip north ignition type, 3 m/s wind speed and 310$^\circ$ wind direction, the MSE value is higher than the standard ConvLSTM model with MSE loss function. This is also reflected in the overestimated fuel density values in the burned cells also presented in the visualization in Figure~\ref{fig:extrapolate}. Figure~\ref{fig:extrapolate} also indicates that the physics-guided model has more stable fuel density predictions across different wind conditions. Especially for the unburned cells, the fuel density values are predicted accurately. On the other hand, for some test samples, the MSE loss based ConvLSTM model is unable to predict the values in unburned cells accurately and has higher fuel density predictions on the perimeter of the fire.

% \begin{figure}[h]
% %\captionsetup[figure]{skip=-15pt}
% \setlength{\belowcaptionskip}{-10pt}
%     \centering
%     \includegraphics[scale=0.3]{images/appendix/extrapolate/pred.eps}
%     \caption{\small \textbf{Individual Predictions}: Predicting at 100$^{th}$ time step with MSE ConvLSTM model and Physics-Guided, physics-guided model. s=speed, d=direction.}
%     \label{fig:extrapolate}
% \end{figure}
% In addition to test set evaluation metrics, we are also interested in the generalization of the model to different ignition types, wind speeds and wind directions. Figure~\ref{fig:msebywind} presents the MSE values for different simulation runs in the test set. The MSE values are represented by the color and differentiated by wind direction (y axis) and wind speed (x axis). We compare the MSE in extrapolation setting when predicting for 50 to 100 seconds (subfigure c and d) and the MSE values when predicting for 0 to 50 seconds (subfigure a and b). We can see that the ConvLSTM model with Physics-Guided loss in the objective function achieves lower MSE. These results, along with the individual prediction results, suggest that predicting fuel density for relatively higher initial wind speeds and wind directions is challenging. Therefore, informing the model learning using physical constraints can enable the ML model to learn better predictions. Despite the physical consistency that we achieve using the reference data and the physics-informed loss terms, fuel density estimation under extreme wind conditions is still a challenge. Moreover, due to a larger number of unburned pixels, there is an imbalance in the contribution of burned cells in the loss term. This results in inaccurate fuel density prediction in the burned area. Solving these challenges will be part of future work.


\subsection{Generalization Performance}

\begin{table}[h]
    \centering
    \scriptsize
    
    \begin{tabular}{p{2cm}llll}
        \hline

        Method & Category &  MSE (0-50 seconds) & MSE (50-100 seconds)\\ \cmidrule(lr){1-4}
        Physics-Guided  & Wind Speed \< 10   & 0.011 & 0.013  \\
        Data-Driven  & Wind Speed \< 10   & 2.635 & 2.525  \\
        Physics-Guided  & Wind Speed \> 10   & 0.031 & 0.036  \\
        Data-Driven  & Wind Speed \> 10   & 3.174 & 3.210  \\
        Physics-Guided  & Ignition Pattern Aerial   & 0.019  & 0.021   \\
        Data-Driven  & Ignition Pattern Aerial    & 2.668 & 2.563   \\
        Physics-Guided  & Ignition Pattern Outward   & 0.001  & 0.004   \\
        Data-Driven  & Ignition Pattern Outward    & 3.165  & 3.145   \\
        Physics-Guided  & Ignition Pattern South   & 0.001 & 0.005   \\
        Data-Driven  & Ignition Pattern South   & 3.182 & 3.034   \\
        Physics-Guided  & Ignition Pattern Inward   & 0.030 & 0.041   \\
        Data-Driven  & Ignition Pattern Inward    & 2.173 & 2.120   \\
        Physics-Guided  & Ignition Pattern North   & 0.002 & 0.004   \\
        Data-Driven  & Ignition Pattern North    & 2.555 & 2.387  \\
        \hline
        \hline
    \end{tabular}
    
    \caption{\small Test set model performance/}
    \label{tab:losses-generalization}
    \vspace{-20pt}
\end{table}











